Speaker Profiling in Multiparty Conversations

In conversational settings, individuals exhibit unique behaviors, rendering a one-size-fits-all approach insufficient for generating responses by dialogue agents. Although past studies have aimed to create personalized dialogue agents using speaker persona information, they have relied on the assumption that the speaker's persona is already provided. However, this assumption is not always valid, especially when it comes to chatbots utilized in industries like banking, hotel reservations, and airline bookings. This research paper aims to fill this gap by exploring the task of Speaker Profiling in Conversations (SPC). The primary objective of SPC is to produce a summary of persona characteristics for each individual speaker present in a dialogue. To accomplish this, we have divided the task into three subtasks: persona discovery, persona-type identification, and persona-value extraction. Given a dialogue, the first subtask aims to identify all utterances that contain persona information. Subsequently, the second task evaluates these utterances to identify the type of persona information they contain, while the third subtask identifies the specific persona values for each identified type. To address the task of SPC, we have curated a new dataset named SPICE, which comes with specific labels. We have evaluated various baselines on this dataset and benchmarked it with a new neural model, SPOT, which we introduce in this paper. Furthermore, we present a comprehensive analysis of SPOT, examining the limitations of individual modules both quantitatively and qualitatively.

==> 7_1_exp_results.tex <==
\subsection{Results}

% \begin{table*}[ht]
% \centering
% \scalebox{0.85}
% {%
% \begin{tabular}{|c|ccc|ccccc|c|}
% \hline
% \multirow{2}{*}{\bf Systems} & \multicolumn{3}{c|}{\bf Persona Discovery} & \multicolumn{6}{c|}{\bf Persona-type Identification} \\ \cline{2-10}
% & \textbf{Precision$^{\dagger}$} & \textbf{Recall$^{\dagger}$} & \textbf{F1$^{\dagger}$} & \textbf{Trait} & \textbf{Likes} & \textbf{Relation} & \textbf{Misc} & \textbf{Occupation} & \textbf{Weighted} \\ \hline
% \textbf{BERT} & 0.17 & 0.72 & 0.27 & 0.48 & 0.0 & 0.09 & 0.24 & 0.05 & 0.24 \\ %\hdashline
% \textbf{DialogXL} & \textbf{0.45} & 0.23 & 0.31 & 0.52 & 0 & 0 & 0 & 0 & 0.18 \\ %\hdashline
% \textbf{Co-GAT} & 0.15 & \textbf{0.94} & 0.27& 0.50 & 0.35 & 0.06 & 0.14 & 0.05 & 0.33 \\ %\hdashline
% \textbf{AGHMN} & 0.43 & 0.14 & 0.21 & 0.56 & 0.58 & 0.38 & 0.26 & 0.25 & 0.48 \\ \hline \hline
% \textbf{\model$_{Base}$} & - & - & - & 0.36 & 0.27 & 0.22 & 0.23 & 0.07 & 0.28 \\ %\hdashline
% \textbf{\model$_{Base+BERT}$} & - & - & - &  0.56 & 0.53 & 0.45 & 0.40 & 0.26 & 0.49 \\ %\hdashline
% \textbf{\model} & 0.30 & 0.50 & \textbf{0.38} & \textbf{0.59} & \textbf{0.6} & \textbf{0.46} & \textbf{0.32} & \textbf{0.28} & \textbf{0.51} \\ \hline
% \end{tabular}%
% }
% \caption{Standalone evaluation ($^{\dagger}$ for the positive class).}%\hl{add whatever ablation is possible}}
% \label{tab:standalone_ph2}
% \end{table*}


% We present the performance of the baseline models and \model\ in this section.
% Note that since two persona types, namely \textit{dislikes} and \textit{education} are very few in number in \dataset,\ we merge them with the \textit{miscellaneous} type.\hl{if you merge, why to specify them separately}
% We first illustrate the results obtained for both the phases when they were evaluated in a standalone fashion, i.e., when ground truth labels were provided to the model for evaluation.
\noindent \textbf{Standalone evaluation.}
We evaluate \model\ for all subtasks of SPC separately and show the results in Table \ref{tab:standalone_ph2} and Table \ref{tab:results-phase3}.
\begin{itemize}[leftmargin=*,noitemsep,topsep=0pt]
    \item \textit{Persona discovery}: We train \model\ as a binary classifier using cross-entropy loss. We obtain $38\%$ F1 score, which is $\sim7\%$ better than the best baseline, DialogXL, as can be seen in Table \ref{tab:standalone_ph2}. The gain in performance can be attributed to the efficient way we use different modules in our architecture to capture different essence of a conversation. It can also be seen that \model\ outperforms the worst performing baseline, AGHMN, by $\sim17\%$. While our model performs the best in terms of F1 score, DialogXL and Co-GAT produce the best performance in terms of precision and recall scores, respectively. On the other hand, \model\ holds a balance between precision and recall to obtain the highest F1 score, which is our metric of choice due to the class imbalance present in our data.
    \item \textit{Persona-type identification}: We use boundary loss \cite{zhang2021deep} to train \model\ for this task. Table \ref{tab:standalone_ph2} shows that \model\ yields a weighted average of $51\%$ F1-score with the maximum score for persona-type \textit{likes}. AGHMN, the best baseline, results in a weighted average of $48\%$ F1-score, which is $\sim3\%$ less than \model. We observe that \model\ achieves the best F1-score for all persona slots showcasing a global dominance of our system. We observe a minimum improvement of $\sim3\%$, $\sim2\%$, $\sim8\%$, $\sim6\%$, and $\sim3\%$ F1-score for the persona slot -- trait, likes, relation, misc, and occupation, respectively, over the existing baselines. It is interesting to observe that our model performs quite well across the persona slots that are dominantly present in our data and consistently decreases for the slots based on their availability in the data.% (c.f. Table \ref{tab:data_stats}). 
    % Further, we show ablation studies based on the incorporation of different modules for the subtask in Appendix Section \ref{app_ablation}%\todo{use \\ref} (Appendix).
    \item \textit{Persona-value extraction}: Using a generative objective, we obtain the results by \model\ for this subtask. Table \ref{tab:results-phase3} demonstrates that \model\ outperforms the baselines by around $1\%$ for all metrics except BLEU 1 and BLEU 3.
\end{itemize}

% following the architecture of \model\ as illustrated in Figure \ref{fig:arch_model1}. 
% The performance of all baselines along with the performance of \model\ is reported in Table \ref{tab:standalone_ph2}. 
% By looking at the F1 score for the positive class, it can be observed that \model\ performs better by atleast $7\%$ than any baseline.
% with an increase of $\sim7\%$ over the best performing baseline, DialogXL.
% We use cross-entropy loss and train \model\ as a binary classifier. We obtain $38\%$ F1 score, which is $\sim7\%$ higher than the best baselines.
% It was observed that {\model} was able to get an F1 score of $36\%$ when no sampling was performed for the persona carrying utterance. In contrast, an F1 score of $38\%$ is obtained if we employ up-sampling in our methodology, indicating that up-sampling to balance the instances of persona carrying and other utterances gives us better results (\sim2\%).\\

% This score is atleast $3\%$ higher than any baseline models. It can also be observed that \model\ gives the best performance for individual persona classes with the maximum score for \textit{likes}.

% \begin{table}[h!]
% \centering
% \subfloat[Persona Discovery ($^{\dagger}$ for the positive class)]{
% \scalebox{0.7}{
% \begin{tabular}{|c|ccc|}
%     \hline
%     \textbf{Systems} & \textbf{Precision$^{\dagger}$} & \textbf{Recall$^{\dagger}$} & \textbf{F1$^{\dagger}$} \\ \hline \hline
%      \textbf{BERT} & 0.17 & 0.72 & 0.27 \\ %\hline
%     \textbf{DialogXL} & \textbf{0.45} & 0.23 & 0.31 \\ %\hline
%     \textbf{Co-GAT} & 0.15 & \textbf{0.94} & 0.27 \\ %\hline
%     \textbf{AGHMN} & 0.43 & 0.14 & 0.21 \\ \hline \hline
%     % \textbf{Ours- without sampling} & 0.27 & 0.52 & 0.36  \\ \hline
%     \textbf{\model} & 0.30 & 0.50 & \textbf{0.38} \\ \hline
% \end{tabular}}
% }\\
% \subfloat[Persona-type Identification]{
% \resizebox{\columnwidth}{!}{
% \begin{tabular}{|c|ccccc|c|}
% \hline
% \textbf{Systems} & \textbf{Trait} & \textbf{Likes} & \textbf{Relation} & \textbf{Misc} & \textbf{Occupation} & \textbf{Weighted} \\ \hline
% \textbf{BERT} & 0.48 & 0.0 & 0.09 & 0.24 & 0.05 & 0.24 \\ %\hdashline
% \textbf{DialogXL} & 0.52 & 0 & 0 & 0 & 0 & 0.18 \\ %\hdashline
% \textbf{Co-GAT} & 0.50 & 0.35 & 0.06 & 0.14 & 0.05 & 0.33 \\ %\hdashline
% \textbf{AGHMN} & 0.56 & 0.58 & 0.38 & 0.26 & 0.25 & 0.48 \\ \hline \hline
% \textbf{\model$_{Base}$} & 0.36 & 0.27 & 0.22 & 0.23 & 0.07 & 0.28 \\ %\hdashline
% \textbf{\model$_{Base+BERT}$} & 0.56 & 0.53 & 0.45 & 0.40 & 0.26 & 0.49 \\ %\hdashline
% \textbf{\model} & \textbf{0.59} & \textbf{0.6} & \textbf{0.46} & \textbf{0.32} & \textbf{0.28} & \textbf{0.51} \\ \hline
% \end{tabular}%
% }}
% \caption{Comparative results for standalone evaluation.}
% \label{tab:standalone_ph2}
% \vspace{-5mm}
% \end{table}

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c||ccc||cccccc|}
\hline
\multirow{2}{*}{\textbf{Systems}} & \multicolumn{3}{c||}{\textbf{\textit{Persona Discovery}}} & \multicolumn{6}{c|}{\textbf{\textit{Persona-type Identification}}} \\ \cline{2-10} 
 & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \textbf{F1} & \multicolumn{1}{c|}{\textbf{Trait}} & \multicolumn{1}{c|}{\textbf{Likes}} & \multicolumn{1}{c|}{\textbf{Rel}} & \multicolumn{1}{c|}{\textbf{Misc}} & \multicolumn{1}{c|}{\textbf{Occ}} & \textbf{Wtd} \\ \hline \hline
\textbf{BERT} & \multicolumn{1}{c|}{0.17} & \multicolumn{1}{c|}{0.72} & 0.27 & \multicolumn{1}{c|}{0.48} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.09} & \multicolumn{1}{c|}{0.24} & \multicolumn{1}{c|}{0.05} & 0.24 \\ \hline
\textbf{DialogXL} & \multicolumn{1}{c|}{\textbf{0.45}} & \multicolumn{1}{c|}{0.23} & 0.31 & \multicolumn{1}{c|}{0.52} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.0} & 0.18 \\ \hline
\textbf{Co-GAT} & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{\textbf{0.94}} & 0.27 & \multicolumn{1}{c|}{0.50} & \multicolumn{1}{c|}{0.35} & \multicolumn{1}{c|}{0.06} & \multicolumn{1}{c|}{0.14} & \multicolumn{1}{c|}{0.05} & 0.33 \\ \hline
\textbf{AGHMN} & \multicolumn{1}{c|}{0.43} & \multicolumn{1}{c|}{0.14} & 0.21 & \multicolumn{1}{c|}{0.56} & \multicolumn{1}{c|}{0.58} & \multicolumn{1}{c|}{0.38} & \multicolumn{1}{c|}{0.26} & \multicolumn{1}{c|}{0.25} & 0.48 \\ \hline \hline
\textbf{\model} & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{0.50} & \textbf{0.38} & \multicolumn{1}{c|}{\textbf{0.59}} & \multicolumn{1}{c|}{\textbf{0.60}} & \multicolumn{1}{c|}{\textbf{0.46}} & \multicolumn{1}{c|}{\textbf{0.32}} & \multicolumn{1}{c|}{\textbf{0.28}} & \textbf{0.51} \\ \hline
\end{tabular}%
}
\caption{Comparative results for standalone evaluation. (P: Precison; R: Recall; Rel: Relationship; Occ: Occupation; Wtd: Weighted F1 score.}
\label{tab:standalone_ph2}
\vspace{-4mm}
\end{table}

% \noindent \textbf{Pipeline Evaluation.} Table \ref{tab-e2e} shows the
% % In the pipeline model, we evaluate {\model} in a back to back fashion. That is, we give \textit{persona discovery} all the dialogues from the entire dataset as the input, whether they contain persona information or not. That is, all the utterances identified as persona carrying \textit{persona discovery} are passed on for \textit{persona type identification} without verification from the ground truth.
% performance obtained by our model along with the baseline scores. For the task of persona discovery, we obtain the same results as standalone due to the same type of input and evaluation strategy (c.f. Table \ref{tab-e2e}(a)). However, in Table \ref{tab-e2e}(b), we observe a performance drop of $\sim8\%$ for the persona-type identification task when compared to the standalone results. This is expected as the erroneous predictions from the first stage may propagate to the second stage. Nevertheless, when compared to the baseline systems, our proposed mechanism gives the best weighted F1-score, with an increase of $\sim3\%$ over the best baseline and $\sim36\%$ over the least performing baseline, BERT. Apart from relation, \model\ performs the best for all persona slots with a performance increase 
% of $\sim8\%$, $\sim7\%$, $\sim5\%$, and $\sim5\%$ for the persona slot trait, likes, misc, and occupation, respectively. These results reinforce our belief that \model\ is able to capture the essence of persona more clearly when compared with the baseline systems.
% % between $\sim5\%$ to $\sim8\%$ F1-score.

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c||ccc||cccccc|}
\hline
\multirow{2}{*}{\textbf{Systems}} & \multicolumn{3}{c||}{\textbf{\textit{Persona Discovery}}} & \multicolumn{6}{c|}{\textbf{\textit{Persona-slot Identification}}} \\ \cline{2-10}
 & \multicolumn{1}{c|}{\textbf{P}} & \multicolumn{1}{c|}{\textbf{R}} & \textbf{F1} & \multicolumn{1}{c|}{\textbf{Trait}} & \multicolumn{1}{c|}{\textbf{Likes}} & \multicolumn{1}{c|}{\textbf{Rel}} & \multicolumn{1}{c|}{\textbf{Misc}} & \multicolumn{1}{c|}{\textbf{Occ}} & \textbf{Wtd} \\ \hline \hline
\textbf{BERT} & \multicolumn{1}{c|}{0.17} & \multicolumn{1}{c|}{0.72} & 0.27 & \multicolumn{1}{c|}{0.12} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.05} & \multicolumn{1}{c|}{0.07} & \multicolumn{1}{c|}{0.0} & 0.07 \\ \hline
\textbf{DialogXL} & \multicolumn{1}{c|}{\textbf{0.45}} & \multicolumn{1}{c|}{0.23} & 0.31 & \multicolumn{1}{c|}{0.33} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.0} & 0.07 \\ \hline
\textbf{Co-GAT} & \multicolumn{1}{c|}{0.15} & \multicolumn{1}{c|}{\textbf{0.94}} & 0.27 & \multicolumn{1}{c|}{0.31} & \multicolumn{1}{c|}{0.26} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{0.07} & \multicolumn{1}{c|}{0.0} & 0.15 \\ \hline
\textbf{AGHMN} & \multicolumn{1}{c|}{0.43} & \multicolumn{1}{c|}{0.14} & 0.21 & \multicolumn{1}{c|}{0.48} & \multicolumn{1}{c|}{0.43} & \multicolumn{1}{c|}{\textbf{0.41}} & \multicolumn{1}{c|}{0.21} & \multicolumn{1}{c|}{0.16} & 0.40 \\ \hline \hline
\textbf{\model} & \multicolumn{1}{c|}{0.30} & \multicolumn{1}{c|}{0.50} & \textbf{0.38} & \multicolumn{1}{c|}{\textbf{0.56}} & \multicolumn{1}{c|}{\textbf{0.50}} & \multicolumn{1}{c|}{0.35} & \multicolumn{1}{c|}{\textbf{0.26}} & \multicolumn{1}{c|}{\textbf{0.21}} & \textbf{0.43} \\ \hline
\end{tabular}%
}
\caption{Comparative results for pipeline evaluation.}
\label{tab-e2e}
\vspace{-4mm}
\end{table}

\noindent \textbf{Pipeline evaluation.} Tables \ref{tab-e2e} and  \ref{tab:results-phase3} show the performance obtained by our model along with the baseline scores. For the task of persona discovery, we obtain the same results as standalone due to the same type of input and evaluation strategies. However, we observe a performance drop of $\sim8\%$ for the persona-type identification task and a drop of at most $\sim6\%$ for the persona-value extraction task when compared to the standalone results. This is expected as the erroneous predictions from the previous stage may propagate to the next stage. Nevertheless, when compared to the baseline systems, our proposed mechanism gives the best score, with an increase of $\sim3\%$ over the best baseline and $\sim36\%$ over the worst performing baseline, BERT, for the former two tasks (c.f. Table \ref{tab-e2e}). Apart from \textit{relation}, \model\ performs the best for all persona slots with a performance increase of $\sim8\%$, $\sim7\%$, $\sim5\%$, and $\sim5\%$ for the persona slot -- trait, likes, misc, and occupation, respectively. While for the last subtaks, we obtain an improvement of $\sim1\%$ over the baselines. Consequently, we establish that \model\ is able to capture the essence of persona more clearly when compared with the baseline systems.
% % between $\sim5\%$ to $\sim8\%$ F1-score.

% {\color{white}.}

% \noindent \textbf{Comparative results.} We evaluate the baselines discussed in Section \ref{sec:baseline} in standalone and pipeline settings. A comparison of the performance of \model\ with the baselines is illustrated in Table \ref{tab:standalone_ph2} for the standalone setting.
% % compares the performance of the baselines with \model\ when they are examined in the standalone setting.
% We observe that \model\ outperforms the baselines by at least $7\%$ for  \textit{persona discovery}. Moreover, \model\ gives a performance boost of $17\%$ over the worst performing baseline, AGHMN. For \textit{persona-type identification}, 
% % We perform experiments for both the phases in standalone and pipeline fashion for all the models. We show the comparative standalone evaluation in Table \ref{tab:standalone_ph2}. 
% % For the task of \textit{persona discovery}, it can be clearly seen that {\model} gives the best performance if we see the F1 score for the positive class. Even without sampling, our model outperforms the baselines by a margin of $\sim5\%$. However, oversampling the data to balance out the negative and positive classes improves the performance by $7\%$ over the baselines.
%  \model\ outperforms the best baseline, AGHMN, by $\sim3\%$ F1 score. In addition, \model\ gives the best performance for individual persona-types with the maximum score for \textit{likes}.
% % followed by \textit{trait},\ \textit{relation},\ \textit{miscellaneous},\ and \textit{occupation}.
% In case of pipeline evaluation, \model\ still performs better than the baselines by atleast $3\%$ with a maximum improvement of $26\%$ for the task of \textit{persona-type identification}.
% % For \textit{persona-type identification} also, our model outperforms the baselines by $3\%$ F1 score. As can be seen in Table \ref{tab:standalone_ph2}, the best performing baseline, AGHMN, gives us a weighted F1 score of $0.48$ while our model outperforms it to give a score of $0.51$. It can also be observed that the highest F1 scores are seen for either the persona class \textit{trait} or \textit{likes}. This is due to their dominance in {\dataset} as can be seen in Figure \ref{fig:slots_dist}.

% \begin{table}[h!]
% \centering
% \subfloat[Persona Discovery ($^{\dagger}$ for the positive class)]{
% \scalebox{0.7}{
% \begin{tabular}{|c|ccc|} \hline
%     \textbf{Systems} & \textbf{Precision}$^{\dagger}$ & \textbf{Recall}$^{\dagger}$ & \textbf{F1}$^{\dagger}$ \\ \hline \hline
%     \textbf{BERT} & 0.17 & 0.72 & 0.27 \\
%     \textbf{DialogXL} & 0.45 & 0.23 & 0.31 \\
%     \textbf{Co-GAT} & 0.15 & 0.94 & 0.27 \\
%     \textbf{AGHMN} & 0.43 & 0.14 & 0.21 \\ \hline \hline
%     \textbf{\model} & 0.30 & 0.50 & 0.38 \\ \hline
% \end{tabular}}
% }\\
% \subfloat[Persona-type Identification]{
% \scalebox{0.6}{
% \begin{tabular}{|c|ccccc|c|} \hline
%      \textbf{Systems} & \textbf{Trait} & \textbf{Likes} & \textbf{Relation} & \textbf{Misc} & \textbf{Occupation} & \textbf{Weighted} \\ \hline \hline
%      \textbf{BERT} & 0.12 & 0.0 & 0.05 & 0.07 & 0.0 & 0.07 \\
%      \textbf{DialogXL} & 0.33 & 0.0 & 0.0 & 0.0 & 0.0 & 0.07 \\
%      \textbf{Co-GAT} & 0.31 & 0.26 & 0.0 & 0.07 & 0.0 & 0.15 \\
%      \textbf{AGHMN} & 0.48 & 0.43 & 0.41 & 0.21 & 0.16 & 0.40 \\ \hline \hline
%      \textbf{\model} & 0.56 & 0.50 & 0.35 & 0.26 & 0.21 & 0.43 \\ \hline
% \end{tabular}
% }}
% \caption{Comparative results for pipeline evaluation.}
% \label{tab-e2e}
% \vspace{-5mm}
% \end{table}

% \begin{table*}[ht]
% \centering
% \scalebox{0.85}
% {%
% \begin{tabular}{|c|ccc|ccccc|c|}
% \hline
% \multirow{2}{*}{\bf Systems} & \multicolumn{3}{c|}{\bf Persona Discovery} & \multicolumn{6}{c|}{\bf Persona-type Identification} \\ \cline{2-10}
% & \textbf{Precision$^{\dagger}$} & \textbf{Recall$^{\dagger}$} & \textbf{F1$^{\dagger}$} & \textbf{Trait} & \textbf{Likes} & \textbf{Relation} & \textbf{Misc} & \textbf{Occupation} & \textbf{Weighted} \\ \hline
% \textbf{BERT} & 0.17 & 0.72 & 0.27 & 0.12 & 0.0 & 0.05 & 0.07 & 0.0 & 0.07 \\ %\hdashline
% \textbf{DialogXL} & \textbf{0.45} & 0.23 & 0.31 & 0.33 & 0 & 0 & 0 & 0 & 0.12 \\ %\hdashline
% \textbf{Co-GAT} & 0.15 & \textbf{0.94} & 0.27 & 0.31 & 0.26 & 0 & 0.07 & 0 & 0.15 \\ %\hdashline
% \textbf{AGHMN} & 0.43 & 0.14 & 0.21 & 0.48 & 0.43 & \bf 0.41 & 0.21 & 0.16 & 0.40 \\ \hline \hline
% \textbf{\model} & 0.30 & 0.50 & \textbf{0.38} & \textbf{0.56} & \textbf{0.50} & 0.35 & \textbf{0.26} & \textbf{0.21} & \textbf{0.43} \\ \hline
% \end{tabular}%
% }
% \caption{ Pipeline evaluation ($^{\dagger}$ for the positive class).}
% \label{tab-e2e}
% \vspace{-5mm}
% \end{table*}

% \begin{table}[h!]
% \centering
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{|l|l|l|l|l|}
% \hline
%  & \textbf{Precision for 1} & \textbf{Recall for 1} & \textbf{F1 for 1} \\ \hline
% \textbf{DialogXL} & \textbf{0.45} & 0.23 & 0.31  \\ \hline
% \textbf{Co-GAT} & 0.15 & \textbf{0.94} & 0.27  \\ \hline
% \textbf{AGHMN} & 0.43 & 0.14 & 0.21 \\ \hline \hline
% \textbf{Ours- without sampling} & 0.27 & 0.52 & 0.36 \\ \hline
% \textbf{Ours- with sampling} & 0.3 & 0.5 & \textbf{0.38} \\ \hline
% \end{tabular}%
% }
% \caption{Standalone evaluation for phase 1}
% \label{tab:standalone_ph1}
% \end{table}


% \begin{table}[h!]
% \centering
% \resizebox{\columnwidth}{!}
% {%
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
%  & \textbf{Trait} & \textbf{Likes} & \textbf{Relation} & \textbf{Misc} & \textbf{Occupation} & \textbf{Weighted} \\ \hline
% \textbf{DialogXL} & 0.52 & 0 & 0 & 0 & 0 & 0.18 \\ \hline
% \textbf{Co-GAT} & 0.5 & 0.35 & 0.06 & 0.14 & 0.05 & 0.33 \\ \hline
% \textbf{AGHMN} & 0.56 & 0.58 & 0.38 & 0.26 & 0.25 & 0.48 \\ \hline \hline
% \textbf{Ours} & \textbf{0.59} & \textbf{0.6} & \textbf{0.46} & \textbf{0.32} & \textbf{0.28} & \textbf{0.51} \\ \hline
% \end{tabular}%
% }
% \caption{Standalone evaluation for phase 2}
% \label{tab:standalone_ph2}
% \end{table}

% \begin{table}[h!]
% \centering
% % \resizebox{0.7\columnwidth}{!}
% {%
% \begin{tabular}{|c|c|c|}
% \hline
% \multirow{2}{*}{} & \textbf{Phase 1} & \textbf{Phase 2} \\ \cline{2-3} 
%  & \textbf{F1 for 1} & \textbf{Weighted} \\ \hline
% \textbf{DialogXL} & 0.31 & 0.12 \\ \hline
% \textbf{Co-GAT} & 0.27 & 0.15 \\ \hline
% \textbf{AGHMN} & 0.21 & 0.40 \\ \hline \hline
% \textbf{Ours} & 0.36 & 0.43 \\ \hline
% \end{tabular}%
% }
% \caption{Pipeline evaluation for phase 1 and 2}
% \label{tab:pipeline}
% \end{table}

\begin{table}[t]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|c||ccccc||ccccc|}
\hline
\multirow{2}{*}{\textbf{Models}} & \multicolumn{5}{c||}{\textbf{Standalone}} & \multicolumn{5}{c|}{\textbf{Pipeline}} \\ \cline{2-11} 
 & \multicolumn{1}{c|}{\textbf{R1}} & \multicolumn{1}{c|}{\textbf{R2}} & \multicolumn{1}{c|}{\textbf{B1}} & \multicolumn{1}{c|}{\textbf{B2}} & \textbf{B3} & \multicolumn{1}{c|}{\textbf{R1}} & \multicolumn{1}{c|}{\textbf{R2}} & \multicolumn{1}{c|}{\textbf{B1}} & \multicolumn{1}{c|}{\textbf{B2}} & \textbf{B3} \\ \hline \hline
\textbf{RNN} & \multicolumn{1}{c|}{26.85} & \multicolumn{1}{c|}{2.28} & \multicolumn{1}{c|}{24.78} & \multicolumn{1}{c|}{1.48} & 0.36 & \multicolumn{1}{c|}{19.64} & \multicolumn{1}{c|}{0.37} & \multicolumn{1}{c|}{18.98} & \multicolumn{1}{c|}{0.36} & 1.12 \\ \hline
\textbf{Transformer} & \multicolumn{1}{c|}{26.02} & \multicolumn{1}{c|}{2.37} & \multicolumn{1}{c|}{23.93} & \multicolumn{1}{c|}{1.54} & 0.58 & \multicolumn{1}{c|}{19.48} & \multicolumn{1}{c|}{0.70} & \multicolumn{1}{c|}{18.82} & \multicolumn{1}{c|}{0.69} & 2.05 \\ \hline
\textbf{PGN} & \multicolumn{1}{c|}{24.40} & \multicolumn{1}{c|}{1.59} & \multicolumn{1}{c|}{23.12} & \multicolumn{1}{c|}{1.08} & 0.36 & \multicolumn{1}{c|}{17.11} & \multicolumn{1}{c|}{0.49} & \multicolumn{1}{c|}{16.13} & \multicolumn{1}{c|}{0.33} & \textbf{9.28} \\ \hline
\textbf{BART} & \multicolumn{1}{c|}{28.93} & \multicolumn{1}{c|}{2.16} & \multicolumn{1}{c|}{\textbf{27.23}} & \multicolumn{1}{c|}{1.51} & 0.36 & \multicolumn{1}{c|}{22.41} & \multicolumn{1}{c|}{\textbf{1.01}} & \multicolumn{1}{c|}{21.37} & \multicolumn{1}{c|}{0.80} & 0.08 \\ \hline
\textbf{T5} & \multicolumn{1}{c|}{15.07} & \multicolumn{1}{c|}{0.0} & \multicolumn{1}{c|}{14.90} & \multicolumn{1}{c|}{2.25} & {\textbf{1.20}} & \multicolumn{1}{c|}{11.62} & \multicolumn{1}{c|}{0.37} & \multicolumn{1}{c|}{11.51} & \multicolumn{1}{c|}{0.36} & 1.12 \\ \hline \hline
\textbf{\model} & \multicolumn{1}{c|}{\textbf{29.51}} & \multicolumn{1}{c|}{\textbf{2.97}} & \multicolumn{1}{c|}{27.16} & \multicolumn{1}{c|}{\textbf{2.27}} & 0.60 & \multicolumn{1}{c|}{\textbf{23.40}} & \multicolumn{1}{c|}{0.60} & \multicolumn{1}{c|}{\textbf{22.12}} & \multicolumn{1}{c|}{\textbf{1.12}} & 0.08 \\ \hline
\end{tabular}%
}
\caption{Comparative results for standalone and pipeline evaluation for \textit{persona-value extraction}.}
\label{tab:results-phase3}
\vspace{-4mm}
\end{table}

==> packages.tex <==
% \usepackage{microtype}
% \usepackage{graphicx}
% \usepackage{multirow}
% \usepackage{arydshln}
% \let\labelindent\relax
% \usepackage{enumitem,colortbl}
% \usepackage{times}
% \usepackage{latexsym}
% \usepackage{subfig}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{soul}
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}

% \definecolor{LightCyan}{rgb}{0.88,1,1}
% \newcommand{\dataset}{\texttt{SPICE}}
% \newcommand{\model}{\texttt{SPOT}}
% \newcommand*{\bfrac}[2]{\genfrac{\lbrace}{\rbrace}{0pt}{}{#1}{#2}}
